Smart Scheduling of Continuous Data-Intensive Workflows with Machine Learning Triggered Execution

To extract value from evergrowing volumes of data, coming from a number of different sources, and to drive decision making, organizations frequently resort to the composition of data processing workflows, since they are expressive, flexible, and scalable. The typical workflow model enforces strict temporal synchronization across processing steps without accounting the actual effect of intermediate computations on the final workflow output. However, this is not the most desirable behavior in a multitude of scenarios. We identify a class of applications for continuous data processing where workflow output changes slowly and without great significance in a short-to-medium time window, thus wasting compute resources and energy with current approaches. To overcome such inefficiency, we introduce a novel workflow model, for continuous and data-intensive processing, capable of relaxing triggering semantics according to the impact input data is assessed to have on changing the workflow output. To assess this impact, learn the correlation between input and output variation, and guarantee correctness within a given tolerated error constant, we rely on Machine Learning. The functionality of this workflow model is implemented in SmartFlux, a middleware framework which can be effortlessly integrated with existing workflow managers. Experimental results indicate we are able to save a significant amount of resources while not deviating the workflow output beyond a small error constant with high confidence level.

==> sections/evaluation-accuracy.tex <==
\begin{figure*}
    \centering

    \subfigure[LRB(5\%) Accuracy] {    
    	\includegraphics[width=0.20\textwidth]{lrb-accuracy-overall-5}
    	\label{fig:accuracy-a}
    }
    \subfigure[LRB(5\%) Precision] {    
    	\includegraphics[width=0.20\textwidth]{lrb-precision-overall-5}
    	\label{fig:accuracy-b}
    }
    \subfigure[LRB(5\%) Recall] {    
    	\includegraphics[width=0.20\textwidth]{lrb-recall-overall-5}
    	\label{fig:accuracy-c}    
    }
    \subfigure[LRB(5\%) F1Score] {    
    	\includegraphics[width=0.20\textwidth]{lrb-f1score-overall-5}
    	\label{fig:accuracy-d}
    }\\    
    \subfigure[LRB(10\%) Accuracy] {    
    	\includegraphics[width=0.20\textwidth]{lrb-accuracy-overall-10}
    	\label{fig:accuracy-e}
    }
    \subfigure[LRB(10\%) Precision] {    
    	\includegraphics[width=0.20\textwidth]{lrb-precision-overall-10}
    	\label{fig:accuracy-f}
    }
    \subfigure[LRB(10\%) Recall] {    
    	\includegraphics[width=0.20\textwidth]{lrb-recall-overall-10}
    	\label{fig:accuracy-g}
    }
    \subfigure[LRB(10\%) F1Score] {    
    	\includegraphics[width=0.20\textwidth]{lrb-f1score-overall-10}
    	\label{fig:accuracy-h}
    }\\
    
    \subfigure[LRB(20\%) Accuracy] {
    	\includegraphics[width=0.20\textwidth]{lrb-accuracy-overall-20}
    	\label{fig:accuracy-i}
    }
    \subfigure[LRB(20\%) Precision] {    
    	\includegraphics[width=0.20\textwidth]{lrb-precision-overall-20}
    	\label{fig:accuracy-j}
    }
    \subfigure[LRB(20\%) Recall] {    
    	\includegraphics[width=0.20\textwidth]{lrb-recall-overall-20}
    	\label{fig:accuracy-k}
    }
    \subfigure[LRB(20\%) F1Score] {    
    	\includegraphics[width=0.20\textwidth]{lrb-f1score-overall-20}
    	\label{fig:accuracy-l}
    }\\
    
    
    \subfigure[AQHI(5\%) Accuracy] {    
    	\includegraphics[width=0.20\textwidth]{aqhi-accuracy-overall-5}
    	\label{fig:accuracy-m}
    }
    \subfigure[AQHI(5\%) Precision] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-precision-overall-5}
    	\label{fig:accuracy-n}
    }
    \subfigure[AQHI(5\%) Recall] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-recall-overall-5}
    	\label{fig:accuracy-o}
    }
    \subfigure[AQHI(5\%) F1Score] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-f1score-overall-5}
    	\label{fig:accuracy-p}
    }
    \\
    
    \subfigure[AQHI(10\%) Accuracy] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-accuracy-overall-10}
    	\label{fig:accuracy-q}
    }
    \subfigure[AQHI(10\%) Precision] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-precision-overall-10}
    	\label{fig:accuracy-r}
    }
    \subfigure[AQHI(10\%) Recall] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-recall-overall-10}
    	\label{fig:accuracy-s}
    }
    \subfigure[AQHI(10\%) F1Score] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-f1score-overall-10}
    	\label{fig:accuracy-t}
    }
	\\

    \subfigure[AQHI(20\%) Accuracy] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-accuracy-overall-20}
    	\label{fig:accuracy-u}
    }
    \subfigure[AQHI(20\%) Precision] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-precision-overall-20}
    	\label{fig:accuracy-v}
    }
    \subfigure[AQHI(20\%) Recall] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-recall-overall-20}
    	\label{fig:accuracy-w}
    }
    \subfigure[AQHI(20\%) F1Score] {    
    	\includegraphics[width=0.2\textwidth]{aqhi-f1score-overall-20}
    	\label{fig:accuracy-x}
    }

    \caption{Accuracy, Precision, Recall, and F1Score for LRB and AQHI with an error bound of 5, 10, and 20\%}
    \label{fig:accuracy}
\end{figure*}

==> sections/model__Joao_SIlva_s_conflicted_copy_2014-12-13_.tex <==
% intro
In this section we describe our workflow model that enables temporal asynchrony by allowing flexible control of the triggering of processing steps based on the predicted impact that observed data patterns in the input have on the workflow result. Our model is specifically designed for continuous processing and data-intensive scenarios where long-lasting workflow applications are regularly feed with raw data from a given source (e.g., network of sensors, Internet, social network, radio telescopes).

Our workflow model inherits from and extends the traditional workflow model~\cite{workflow-survey-2005} where strict temporal synchronization is enforced. As our target is data-intensive applications, we define that, in our model, the worflow underlying data must be shared, among processing steps, through distributed Key-Value storage, since we perform specific analysis and processing for this type of storage. Most workflow models, in contrast, only rely on files to store and share the data, which cannot achieve the same scalability and flexibility, hence we believe this assumption to fit many, if not most, large scale data processing scenarios.

In particular, what differentiates and demarcates our model from the other typical DAG workflows is the triggering semantics: a processing step A, in a workflow D, is not necessarily triggered for execution immediately, when all its predecessors A' ($A' \prec_D A$) have finished their execution. Instead, A should only be triggered as soon as all predecessor steps A' have completed at least one execution and have, also, carried out a sufficient (or significant) level of changes on the underlying database 
that comply with certain QoD requirements. This way, a processing step can be re-executed several times without triggering the execution of successor nodes; i.e., the triggering of steps is guided by data changes and not exclusively by the end of single execution of predecessor nodes, as it usually happens in the regular workflow model. This behavior is similar to that of Google Percolator~\cite{Peng:2010:LIP:1924943.1924961}.


The QoD that a processing step needs to comply with corresponds to the impact that its input is targeted to have (which comes from the generated output of predecessor steps), according to a certain defined metric. By turn, the target impact on input corresponds to the input necessary, in terms of quantity and quality (or significance), for reaching a threshold that specifies the maximum deviation of the output tolerated for that step. This output deviation in a step can be seen as an error introduced by delaying and skipping its (re-)execution, as opposed to the synchronous model. In return, this delay and skip save resources from being wastefully engaged. Following, we describe the metrics to calculate the input impact and the output error.


\subsection{Input Impact}


The input impact of a processing step is a metric that captures the amount and magnitude of changes performed on its associated data container (e.g., a column or a set of columns) in relation to a previous state, corresponding to the latest execution of that step. In distributed Key-Value stores, like the columnar-oriented HBase and Cassandra, data containers may consist of keyspaces, tables, columns (including hierarchical columns), rows, or any combination of these, and it is usually trivial, through simple get-put interfaces, to capture the scope of update operations in terms of affected containers; i.e., there is no need to deal with wider-scope queries possibly containing complex aggregate operations. We refer to an element in a data container as a (multi-dimensional) Key-Value pair.

Every time new data updates are performed on a data container associated with a processing step, the input impact is calculated on the fly (without needing to take snapshots of containers in previous states) based on the current and new data that is being updated. Soon after, the assessed impact on a wave is accumulated with the impact measured for previous waves that occurred after the execution of the associated step. Since all steps are potentially not executed at the same wave, the input impact is only calculated when its predecessor steps have generated output, which will possibly not happen in every wave.

Although for the future we plan to provide an expressive high-level language (e.g., LUA~\cite{SPE:SPE26}) to define arbitrary functions to capture the impact of changes in a data container, we now offer three different and general functions that can serve well a wide set of scenarios. They are described as follows.

\begin{equation}
\label{eq:input-impact-1}
\iota=\sum\limits_{i=1}^m |x_i - x_i'|
\end{equation}

\mymark{fix line below}
Equation~\ref{eq:input-impact-1}                      , where $x_i$ is the updated state of the ith element and $x_i'$ its latest state, and $m$ is the number of modified elements in the respective data container)


\begin{equation}
\label{eq:input-impact-2}
\iota=\sum\limits_{i=1}^m |x_i - x_i'|
\end{equation}

Equation~\ref{eq:input-impact-2}



\begin{equation}
\label{eq:input-impact-3}
\iota=\sum\limits_{i=1}^m |x_i - x_i'|
\end{equation}

Equation~\ref{eq:input-impact-3}


\mymark{ESPECIFICAR DIFERENÇAS ENTRE FORMULAS}


%%Since the input data of intermediate and output steps depend on the input data of input steps (i.e., the ones that are supplied with data from external sources), the input impact only needs to be calculated, in most of the cases, for the input steps of the workflow. 
%This impact of the input, %whether it is solely the input fed to the workflow or the input 
%fed to each single processing step, is measured through the tridimensional vector $\iota_o = (\sigma, \nu, \delta)$, where $\sigma$ is the number of updates performed on data container $o$, $\nu$ is the maximum allowed stdeviation of a single item in $o$, and $\delta$ is the sum of all diffs on $o$ between updated items and their latest state ($\sum\limits_{i=1}^m |x_i - x_i'|$, where $x_i$ is the updated state of the ith element and $x_i'$ its latest state, and $m$ is the number of modified elements in the respective data container). *** corrigir linha anterior ***).      



\subsection{Output Error}


The output error of a processing step is a metric that attempts to measure the cost penalty (or impact) of postponing its executions. Each time a step is not executed at a given wave of data, it incurs a certain error that can be translated as the cost of the changes that were missed in the respective data container; hence, if a step is always executed at each wave of data the error is zero. This output error, denoted by $\varepsilon$, is calculated through Equation~\ref{eq:error}, where $x_i$ is the updated state of the ith element and $x_i'$ its latest state, $m$ the number of modified elements, and $n$ the total number of elements in the respective data container.

\begin{equation}
\label{eq:error}
\varepsilon=\frac{\sum\limits_{i=1}^m |x_i - x_i'| \times m}{\sum\limits_{i=1}^n x_i' \times n}
%\varepsilon=\sum\limits_{i=1}^m |x_i - x_i'| \times m / (\sum\limits_{i=1}^n x_i' \times n)
\end{equation}


For each output processing step, the output error $\varepsilon$ must be bounded to guarantee a certain level of correctness and usefulness in the result of the workflow. However, output of intermediate steps can also be bounded so that intermediate results are not much  deviated in relation to the normal execution of the synchronous model. During a period of normal execution, we attempt to learn statistical behavior of the errors for different impacts of input given to processing steps (elaborated in the next section).


%*** este modelo consegue perceber quando há execuçõoes consecutivas que se anulam.  ***

\subsection{Prototypical Scenario}

\begin{figure}
    \includegraphics[width=\columnwidth]{temperature-evolution}
    \caption{Temperature evolution hour by hour for a day in Amazon rainforest}
    \label{fig:temperature-evolution}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{fire-forecast-workflow}
	\caption{Use-case scenario of continuous and incremental workflow processing: fire risk assessment}
	\label{fig:fire-forecast-workflow}
\end{figure}


Figure~\ref{fig:fire-forecast-workflow} ......

==> sections/related-work.tex <==


This section reviews relevant proposed solutions, within the current state-of-the-art, that intersect the main topics approached in this paper. In the workflow domain, popular systems include: DAGMan, Pegasus, Taverna, Dryad, Kepler, Triana, Galaxy~\cite{WMS-survey-2015}.
%WMSs for Hadoop also started to arise like Oozie, Azkaban,\footurl{http://sna-projects.com/azkaban/} and Cascading,\footurl{http://www.cascading.org}.
Next, we describe in more detail the related work that is the closest to our work.

%\cite{springerlink:10.1007/978-1-84628-757-2_22}
%\cite{DBLP:conf/ssdbm/MissierSOTNDWOG10}
%\cite{Isard:2007:DDD:1272996.1273005}
%\cite{10.1109/SSDM.2004.1311241}





%First, we describe general and e-science data/work ow systems. Next, we focus on solutions for incremental processing.


%\subsection{Workflows}
%DAGMan \cite{springerlink:10.1007/978-1-84628-757-2_22} is one of the early workflow languages in e-science. It interprets and manages text descriptions of jobs comprising DAGs. DAGMan accounts for job dependencies, allows pre- and post-processing scripts for each vertex and reissues failed jobs. Being a meta-scheduler, it relies on the centralized Condor workload management system for scheduling. Pegasus \cite{Lee:2009:AWP:1656309.1656311} extends DAGMan in order to allow mapping of workflows jobs on distributed resources and from the description of computation tasks, it performs the necessary data transfers among sites. Pegasus aims at optimizing workflow performance and reliability by scheduling to appropriate resources but there are no QoD guarantees on continuous processing or data flow, and no data sharing.

%Taverna \cite{DBLP:conf/ssdbm/MissierSOTNDWOG10} is heavily used in bioinformatics. It is a WMS with interoperability support for a multitude of execution environments and data formats. Data sources and data links are considered as first entities in the dataflow language. Execution can be placed remotely on a large list of resources but without cross-site distribution and no QoD is enforced.

%Dryad \cite{Isard:2007:DDD:1272996.1273005} executes DAGs explicitly created via an imperative API. It includes composition of operators\slash operations and enabled new ones to be defined, allowing for graph and vertex merger. It allows the construction of computation pipelines spanning across a cluster. It has been integrated with LINQ data query capabilities in .NET languages. It has support for channels of shared mutable data.

%Kepler \cite{10.1109/SSDM.2004.1311241} is a solution for managing scientific workflows. It was designed to help scientists and other inexpert computer users to create, execute, and share models and analyses, thereby including a set of features for reducing the inherent complexity of deploying workflows in various computing environments. Other option is Triana \cite{TaylorTriana-2007}, a decade proven visual programming environment, focusing on minimum effort, that allows users to compose applications from programming components (drawn from a large library on text, signal and image processing) by drag and drop into a workspace, and connecting them in a workflow graph.


%\subsection{Incremental Processing}
MapReduce (MR) \cite{Dean:2004:MSD:1251254.1251264} was first created for reverse index creation and page ranking. It forces programmers to obey a strict model that is different from those used for application logic. However, the automatic parallelization and fault-tolerance features made it powerful and led to the development of the open-source solution Hadoop \cite{White:2009:HDG:1717298}. WMSs for Hadoop, like Oozie, started to arise, e.g., Azkaban,\footurl{http://sna-projects.com/azkaban/}%~\cite{azkaban}
 Cascading.\footurl{http://www.cascading.org}~\cite{cascading}

More modern functionality in MR such as supporting social networks and data analytics are extremely cumbersome to code as a giant set of interdependent MR programs. Reusability is thus very limited. To amend this, DAG-like (workflow) platforms started to emerge on top of MR, such as Apache Tez\footurl{https://tez.apache.org/}%~\cite{tez}
 and Pig\cite{Olston:2008:PLN:1376616.1376726}. The Apache Pig platform eases creation of data analysis programs. The Pig Latin language combines imperative-like script language (foreach, load, store) with SQL-like operators (group, filter). Scripts are compiled into Java programs linked to Map Reduce libraries.
%An example of productivity and reusability is a word counting script with 6 lines of code.
The Hive \cite{Thusoo09hive-a} warehouse reinstates fully declarative SQL-like languages (HiveQL) over data in tables (stored as files in an HDFS directory). Queries are compiled into MR jobs to be executed on Hadoop. SCOPE \cite{Chaiken:2008:SEE:1454159.1454166} takes a similar approach to scripting but targeting Dryad \cite{Isard:2007:DDD:1272996.1273005} for its execution engine.

To avoid recreating web indexes from scratch after each web crawl, Google Percolator \cite{Peng:2010:LIP:1924943.1924961} performs incremental processing on top of BigTable, replacing batch processing of MR. It provides row and table-wide transactions, snapshot isolation, with locks stored in special Bigtable columns. Notify columns are set when rows are updated, with several threads scanning them. Applications are sets of custom-coded observers. Although it scales better than MR, it has 30-fold resource overhead over traditional RDBMS. Nova \cite{Olston:2011:NCP:1989323.1989439} is similar but has no latency goals, accumulating many new inputs and processing them lazily for throughput. Moreover, Nova provides data processing abstraction through Pig Latin; and supports stateful continuous processing of evolving data sets.

Yahoo CBP \cite{Logothetis:2010:SBP:1807128.1807138} aims at greater expressiveness by specifying incremental processing as dataflows with explicit mention when computation stages are stateless or stateful. Input is split by determining membership in frames of new records, allowing grouping input to reduce messaging.
%Thus, as a result of a partial web crawl, a new input frame is processed. For stateful stages, translator functions combine data from new frames with existing state.
CBP provides primitives for explicit control flow and synchronize execution of multiple inputs. It requires an extended MR implementation and some explicit programming to use a QoD-enabled dataflow.

Nectar \cite{Gunda:2010:NAM:1924943.1924949} for Dryad links data and the computation that generated it as unified hybrid cacheable element. On programs reruns, Nectar replaces results with cached data. Dryad programs need to be enhanced with cache management calls that check and update the cache server. This is transparently done in InCoop \cite{Bhatotia:2011:IMI:2038916.2038923}, which does caching for MR applications. Map, combine and reduce phase results are stored and memoized.
%A new memorization-aware scheduler is used to repeat tasks where cached output is already stored, reducing data transfers that still cause overhead even if re-computation is avoided.
Somehow like \name, this project attempts to reduce the number of executions; however, it implies that the input\slash output datasets are repeated or intersected among each other, whereas the QoD model fits a broader range of scenarios.

In \cite{asyncr_olston}, the authors present a formal programming and scheduling model for defining temporal asynchrony in workflows. The workflow vertices consist of operators that process data, and data channels, which are pathways through which data flows between operators. These operators have signatures that describe the types and consistency of the blocks (i.e., the atomic units of data) accepted as input and returned as output. Data channels have a representation of time to a relation snapshot, with an interval of validity, which are used to enforce consistency invariants. These constraints, types of blocks permitted on output, freshness and consistency bounds, are then used by the scheduler which produces minimal-cost execution plans. This project shares our goals of exploring and providing non ad-hoc solutions for introducing asynchronous behavior in workflows, however, it does not account with the volume, relevance or impact of modifications of the data given as input to each workflow step.

In~\cite{DBLP:journals/jisa/EstevesSV13}, authors propose a DAG model where task triggering is based on 3 user-defined constraints: i) the time to trigger a task; ii) the number of updates on the data; and iii) the magnitude of the updates. This allows flexible data-based execution, however i) it is difficult to manually set a combination of constraints in a workflow in order to keep the error  within manageable levels;  and ii) no reasoning is performed about the impact computations have on varying the output. Thus, their model is not usable for scenarios where the freshness of the results needs to be guaranteed (like it is achievable with \name).


% STREAM PROCESSING E LOAD SHEDDING
%Further, it is important to note that \name is not a stream processing system, like Apache Storm\cite{Toshniwal:2014:STO:2588555.2595641} or Spark Streaming [3]. Like other typical WMS, OOzie (the engine behind \name) is triggered by time (frequency) and data availability, which are discrete events in time, and do not rely on sliding windows (as stream processing does). Besides, data is accumulated and persisted in WMS across processing steps, which does not happen in stream processing systems, where data is mostly kept in volatile memory. Continuous processing in the context of this work means that the same aggregated computation (workflow) is executed multiple times over ("non-contiguous") time, and does not mean that workflows are uninterruptedly receiving new input data (like stream processing engines).
Further, it is important to note that we do not discard any data, like it happens in load shedding~\cite{Tatbul:2007:SFE:1325851.1325873}. In load shedding, a fraction of the input data is shed to alleviate overloaded servers and preserve low latency for query results. Contrarily to discarding data, we accumulate it up to the point where it causes significant changes on the output of the workflow. The observed errors happen not because we are making computations with incomplete data, but because we are not performing the computations and generating new output (i.e., errors come from stale data in the output).

There has also been a recent effort to enable approximate processing in data processing systems (e.g., MapReduce, Stream Processing) in order to reduce latency (and possibly resource usage). However, these systems usually only target specific aggregation operators (e.g., sum, count) in structured languages~\cite{Goiri:2015:ABA:2694344.2694351,agarwal:2013:bqb:2465351.2465355,Agarwal:2014:KYW:2588555.2593667}. In our work, we provide approximate results for general-purpose computations; i.e., we are agnostic to the code that is running on each processing step and solely observe the data that is inputted and its effect on modifying the output. Effectively learning the correlation between input and output allows us to bound the error and give guarantees about the correctness of the results. This makes \name unique.


